D-meson semileptonic decays to pseudoscalars from four-flavor lattice QCD

We present lattice-QCD calculations of the hadronic form factors for the semileptonic decays $D\to\pi\ell\nu$, $D\to K\ell\nu$, and $D_s\to K\ell\nu$. Our calculation uses the highly improved staggered quark (HISQ) action for all valence and sea quarks and includes $N_f=2+1+1$ MILC ensembles with lattice spacings ranging from $a\approx0.12$ fm down to $0.042$ fm. At most lattice spacings, an ensemble with physical-mass light quarks is included. The HISQ action allows all the quarks to be treated with the same relativistic light-quark action, allowing for nonperturbative renormalization using partial conservation of the vector current. We combine our results with experimental measurements of the differential decay rates to determine $|V_{cd}|^{D\to\pi}=0.2238(11)^{\rm Expt}(15)^{\rm QCD}(04)^{\rm EW}(02)^{\rm SIB}[22]^{\rm QED}$ and $|V_{cs}|^{D\to K}=0.9589(23)^{\rm Expt}(40)^{\rm QCD}(15)^{\rm EW}(05)^{\rm SIB}[95]^{\rm QED}$ This result for $|V_{cd}|$ is the most precise to date, with a lattice-QCD error that is, for the first time for the semileptonic extraction, at the same level as the experimental error. Using recent measurements from BES III, we also give the first-ever determination of $|V_{cd}|^{D_s\to K}=0.258(15)^{\rm Expt}(01)^{\rm QCD}[03]^{\rm QED}$ from $D_s\to K \ell\nu$. Our results also furnish new Standard Model calculations of the lepton flavor universality ratios $R^{D\to\pi}=0.98671(17)^{\rm QCD}[500]^{\rm QED}$, $R^{D\to K}=0.97606(16)^{\rm QCD}[500]^{\rm QED}$, and $R^{D_s\to K}=0.98099(10)^{\rm QCD}[500]^{\rm QED}$, which are consistent within $2\sigma$ with experimental measurements. Our extractions of $|V_{cd}|$ and $|V_{cs}|$, when combined with a value for $|V_{cb}|$, provide the most precise test of second-row CKM unitarity, finding agreement with unitarity at the level of one standard deviation.

==> D-meson_semileptonic_decays_with_highly_improved_staggered_quarks/Tables/bare_mq.tex <==
\begin{tabular}{cc@{\hspace{0.75em}}lll@{\hspace{0.75em}}lll}
\hline\hline
$\approx a$ & $m_l/m_s$ & $(am_l)^{\rm sea}$ & $(am_s)^{\rm sea}$ & $(am_c)^{\rm sea}$ & $(am_l)^{\rm valence}$ & $(am_s)^{\rm valence}$ & $(am_h)^{\rm valence}$ \\
\hline
0.12        & 1/27      & 0.001907           & 0.05252            & 0.6382             & $(am_l)^{\rm sea}$ & $(am_s)^{\rm sea}$ &\{0.5744, 0.6382, 0.8935\} \\[2pt]
% \hline
0.088       & 1/27      & 0.0012             & 0.0363             & 0.432              & $(am_l)^{\rm sea}$ & $(am_s)^{\rm sea}$ &\{0.389, 0.432, 0.648, 0.864\} \\
0.088       & 1/10      & 0.00363            & 0.0363             & 0.43               & $(am_l)^{\rm sea}$ & $(am_s)^{\rm sea}$ &\{0.389, 0.432, 0.648, 0.864\} \\[2pt]
% \hline
0.057       & 1/27      & 0.0008             & 0.022              & 0.26               & $(am_l)^{\rm sea}$ & $(am_s)^{\rm sea}$ &\{0.257, 0.286, 0.572\} \\
0.057       & 1/10      & 0.0024             & 0.024              & 0.286              & $(am_l)^{\rm sea}$ & $(am_s)^{\rm sea}$ &\{0.257, 0.286, 0.572\} \\
0.057       & 1/5       & 0.0048             & 0.024              & 0.286              & $(am_l)^{\rm sea}$ & $(am_s)^{\rm sea}$ &\{0.257, 0.286, 0.572\} \\[2pt]
% \hline
0.042       & 1/5       & 0.00316            & 0.0158             & 0.188              & 0.00311            & 0.01555            &\{0.164, 0.1827, 0.365\} \\
\hline\hline
\end{tabular}

==> D-meson_semileptonic_decays_with_highly_improved_staggered_quarks/Tables/d2k_vcs_zexpansion_fits.tex <==
\begin{tabular}{c|c|c|c}
$\DK$ & LQCD only & Joint LQCD and Expt & Expt only \\
\hline\hline
$a_0 \equiv b_0$ & $0.7452(31)$ & $0.7450(31)$ & $0.7246(26)$\\
$a_1$ & $-0.948(97)$ & $-1.036(73)$ & $-1.049(89)$\\
$a_2$ & $0.14(40)$ & $0.18(73)$ & $0.10(92)$\\
$a_3$ & $0.07(12)$ & $-0.03(1.00)$ & $-0.03(1.00)$\\
$b_1$ & $0.776(62)$ & $0.772(66)$ & $-$\\
$b_2$ & $0.14(34)$ & $0.08(56)$ & $-$\\
$b_3$ & $0.03(13)$ & $-0.02(99)$ & $-$\\
\hline\hline
\end{tabular}


==> D-meson_semileptonic_decays_with_highly_improved_staggered_quarks/Tables/d2k_zexpansion_fit.tex <==
\begin{tabular}{cccccccc}
$\DK$ & $a_0 \equiv b_0$ & $a_1$ & $a_2$ & $a_3$ & $b_1$ & $b_2$ & $b_3$\\
 & 0.7452(31) & -0.948(97) & 0.14(40) & 0.07(12) & 0.776(62) & 0.14(34) & 0.03(13)\\
\hline
 & 1.0000 & -0.0332 & 0.0747 & -0.0201 & 0.7753 & 0.4920 & -0.0189\\
 &  & 1.0000 & 0.3272 & -0.1586 & -0.0909 & -0.1090 & 0.0420\\
 &  &  & 1.0000 & -0.7543 & 0.2071 & 0.2565 & 0.1457\\
 &  &  &  & 1.0000 & -0.0594 & -0.1119 & -0.2259\\
 &  &  &  &  & 1.0000 & 0.9087 & 0.1012\\
 &  &  &  &  &  & 1.0000 & 0.2126\\
 &  &  &  &  &  &  & 1.0000\\
\end{tabular}


==> D-meson_semileptonic_decays_with_highly_improved_staggered_quarks/Tables/d2pi_vcd_zexpansion_fits.tex <==
\begin{tabular}{c|c|c|c}
$\Dpi$ & LQCD only & Joint LQCD and Expt & Expt only \\
\hline\hline
$a_0 \equiv b_0$ & $0.6300(51)$ & $0.6306(47)$ & $0.1426(17)$\\
$a_1$ & $-0.610(99)$ & $-0.574(83)$ & $-0.157(45)$\\
$a_2$ & $-0.20(30)$ & $-0.009(393)$ & $-0.15(32)$\\
$a_3$ & $0.30(19)$ & $0.32(94)$ & $0.12(94)$\\
$b_1$ & $0.330(51)$ & $0.379(52)$ & $-$\\
$b_2$ & $-0.31(25)$ & $0.22(36)$ & $-$\\
$b_3$ & $-1.90(39)$ & $-0.54(84)$ & $-$\\
\hline\hline
\end{tabular}


==> D-meson_semileptonic_decays_with_highly_improved_staggered_quarks/Tables/d2pi_zexpansion_fit.tex <==
\begin{tabular}{cccccccc}
$\Dpi$ & $a_0 \equiv b_0$ & $a_1$ & $a_2$ & $a_3$ & $b_1$ & $b_2$ & $b_3$\\
 & 0.6300(51) & -0.610(99) & -0.20(30) & 0.30(19) & 0.330(51) & -0.31(25) & -1.90(39)\\
\hline
 & 1.0000 & 0.5670 & 0.5189 & -0.2018 & 0.7547 & 0.3473 & 0.0861\\
 &  & 1.0000 & 0.8912 & -0.2826 & 0.5148 & 0.2529 & 0.0747\\
 &  &  & 1.0000 & -0.1482 & 0.5082 & 0.2782 & 0.1162\\
 &  &  &  & 1.0000 & -0.1728 & -0.0496 & 0.0354\\
 &  &  &  &  & 1.0000 & 0.8277 & 0.6066\\
 &  &  &  &  &  & 1.0000 & 0.9442\\
 &  &  &  &  &  &  & 1.0000\\
\end{tabular}


==> D-meson_semileptonic_decays_with_highly_improved_staggered_quarks/Tables/d2x_zexpansion_correlations.tex <==
\begin{tabular}{ccccccc ccccccc ccccccc}
$\Dpi$ & & & & & & & $\DK$ & & & & & & & $\DsK$ & & & & & & & \\
$a_0 \equiv b_0$ & $a_1$ & $a_2$ & $a_3$ & $b_1$ & $b_2$ & $b_3$ &$a_0 \equiv b_0$ & $a_1$ & $a_2$ & $a_3$ & $b_1$ & $b_2$ & $b_3$ &$a_0 \equiv b_0$ & $a_1$ & $a_2$ & $a_3$ & $b_1$ & $b_2$ & $b_3$\\
\hline
$1.0000$ & $0.5670$ & $0.5189$ & $-0.2018$ & $0.7547$ & $0.3473$ & $0.0861$ & $0.3219$ & $0.0497$ & $0.0635$ & $-0.0439$ & $0.1897$ & $0.1158$ & $-0.0540$ & $0.2342$ & $0.1305$ & $0.1157$ & $-0.0273$ & $0.1810$ & $0.1459$ & $0.1002$\\
 & $1.0000$ & $0.8912$ & $-0.2826$ & $0.5148$ & $0.2529$ & $0.0747$ & $0.1159$ & $0.0559$ & $0.1385$ & $-0.1328$ & $0.1625$ & $0.1704$ & $-0.1148$ & $-0.0037$ & $0.4332$ & $0.3713$ & $0.0198$ & $-0.0341$ & $-0.0351$ & $-0.0284$\\
 &  & $1.0000$ & $-0.1482$ & $0.5082$ & $0.2782$ & $0.1162$ & $0.1313$ & $0.0438$ & $0.1916$ & $-0.0885$ & $0.2166$ & $0.2197$ & $-0.0308$ & $0.0350$ & $0.2987$ & $0.2781$ & $0.0601$ & $-0.0071$ & $-0.0297$ & $-0.0325$\\
 &  &  & $1.0000$ & $-0.1728$ & $-0.0496$ & $0.0354$ & $-0.0115$ & $-0.0907$ & $0.0014$ & $0.2782$ & $0.0787$ & $0.1182$ & $0.0639$ & $0.0529$ & $0.0228$ & $0.0638$ & $0.1488$ & $0.0634$ & $-0.0154$ & $-0.0969$\\
 &  &  &  & $1.0000$ & $0.8277$ & $0.6066$ & $0.1858$ & $0.1995$ & $0.1837$ & $-0.1531$ & $0.1637$ & $0.1608$ & $0.0996$ & $0.2393$ & $0.0457$ & $0.0571$ & $0.0266$ & $0.2161$ & $0.1520$ & $0.0425$\\
 &  &  &  &  & $1.0000$ & $0.9442$ & $0.0846$ & $0.2589$ & $0.2257$ & $-0.1766$ & $0.1439$ & $0.1970$ & $0.2436$ & $0.1943$ & $0.0190$ & $0.0411$ & $0.0403$ & $0.1979$ & $0.1480$ & $0.0299$\\
 &  &  &  &  &  & $1.0000$ & $0.0226$ & $0.2597$ & $0.2111$ & $-0.1572$ & $0.1088$ & $0.1743$ & $0.2784$ & $0.1524$ & $0.0032$ & $0.0261$ & $0.0512$ & $0.1659$ & $0.1280$ & $0.0200$\\
 &  &  &  &  &  &  & $1.0000$ & $-0.0332$ & $0.0747$ & $-0.0201$ & $0.7753$ & $0.4920$ & $-0.0189$ & $0.2613$ & $0.1817$ & $0.1423$ & $-0.1223$ & $0.1642$ & $0.0590$ & $-0.0293$\\
 &  &  &  &  &  &  &  & $1.0000$ & $0.3272$ & $-0.1586$ & $-0.0909$ & $-0.1090$ & $0.0420$ & $0.0715$ & $0.0236$ & $-0.0442$ & $-0.1656$ & $0.0458$ & $0.0377$ & $0.0266$\\
 &  &  &  &  &  &  &  &  & $1.0000$ & $-0.7543$ & $0.2071$ & $0.2565$ & $0.1457$ & $-0.0938$ & $0.1078$ & $0.0219$ & $-0.2929$ & $-0.1126$ & $-0.1094$ & $-0.0790$\\
 &  &  &  &  &  &  &  &  &  & $1.0000$ & $-0.0594$ & $-0.1119$ & $-0.2259$ & $0.1727$ & $-0.0470$ & $0.0700$ & $0.3279$ & $0.1515$ & $0.0836$ & $-0.0062$\\
 &  &  &  &  &  &  &  &  &  &  & $1.0000$ & $0.9087$ & $0.1012$ & $0.2751$ & $0.2429$ & $0.2479$ & $-0.0663$ & $0.1986$ & $0.0374$ & $-0.1217$\\
 &  &  &  &  &  &  &  &  &  &  &  & $1.0000$ & $0.2126$ & $0.2038$ & $0.2315$ & $0.2517$ & $-0.0060$ & $0.1481$ & $-0.0029$ & $-0.1604$\\
 &  &  &  &  &  &  &  &  &  &  &  &  & $1.0000$ & $-0.1959$ & $-0.1108$ & $-0.0868$ & $0.1128$ & $-0.1256$ & $-0.0562$ & $0.0179$\\
 &  &  &  &  &  &  &  &  &  &  &  &  &  & $1.0000$ & $0.1825$ & $0.2612$ & $-0.0266$ & $0.8467$ & $0.5197$ & $0.0973$\\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  & $1.0000$ & $0.9274$ & $-0.2432$ & $0.1899$ & $0.1915$ & $0.1180$\\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & $1.0000$ & $-0.0514$ & $0.3243$ & $0.3065$ & $0.1764$\\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & $1.0000$ & $-0.0551$ & $-0.1580$ & $-0.2098$\\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & $1.0000$ & $0.8344$ & $0.4260$\\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & $1.0000$ & $0.8442$\\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & $1.0000$\\
\end{tabular}


==> D-meson_semileptonic_decays_with_highly_improved_staggered_quarks/Tables/ds2k_vcd_zexpansion_fits.tex <==
\begin{tabular}{c|c|c|c}
$\DsK$ & LQCD only & Joint LQCD and Expt & Expt only \\
\hline\hline
$a_0 \equiv b_0$ & $0.6307(20)$ & $0.6306(20)$ & $0.164(18)$\\
$a_1$ & $-0.562(65)$ & $-0.557(72)$ & $-0.14(29)$\\
$a_2$ & $-0.19(20)$ & $-0.20(42)$ & $-0.03(98)$\\
$a_3$ & $0.33(29)$ & $0.04(98)$ & $0.008(1.000)$\\
$b_1$ & $0.347(27)$ & $0.346(35)$ & $-$\\
$b_2$ & $0.44(18)$ & $0.45(30)$ & $-$\\
$b_3$ & $-0.21(43)$ & $-0.11(96)$ & $-$\\
\hline\hline
\end{tabular}


==> D-meson_semileptonic_decays_with_highly_improved_staggered_quarks/Tables/ds2k_zexpansion_fit.tex <==
\begin{tabular}{cccccccc}
$\DsK$ & $a_0 \equiv b_0$ & $a_1$ & $a_2$ & $a_3$ & $b_1$ & $b_2$ & $b_3$\\
 & 0.6307(20) & -0.562(65) & -0.19(20) & 0.33(29) & 0.347(27) & 0.44(18) & -0.21(43)\\
\hline
 & 1.0000 & 0.1825 & 0.2612 & -0.0266 & 0.8467 & 0.5197 & 0.0973\\
 &  & 1.0000 & 0.9274 & -0.2432 & 0.1899 & 0.1915 & 0.1180\\
 &  &  & 1.0000 & -0.0514 & 0.3243 & 0.3065 & 0.1764\\
 &  &  &  & 1.0000 & -0.0551 & -0.1580 & -0.2098\\
 &  &  &  &  & 1.0000 & 0.8344 & 0.4260\\
 &  &  &  &  &  & 1.0000 & 0.8442\\
 &  &  &  &  &  &  & 1.0000\\
\end{tabular}


==> D-meson_semileptonic_decays_with_highly_improved_staggered_quarks/Tables/form_factor_comparsion.tex <==
\begin{tabular}{lllll}
\hline
process & collaboration &   $f_0(0)$ & $f_0(q^2_{\rm max})$ & $f_+(q^2_{\rm max})$ \\
\hline
   $\Dpi$ &     FNAL/MILC & 0.6300(51) &           1.2783(61) &            3.119(57) \\
   $\Dpi$ &       ETMC 17 &  0.612(35) &            1.134(49) &            2.130(96) \\
    \hline
    $\DK$ &     FNAL/MILC & 0.7452(31) &           1.0240(21) &            1.451(17) \\
    $\DK$ &      HPQCD 22 & 0.7441(40) &           1.0136(36) &            1.462(16) \\
    $\DK$ &      HPQCD 21 & 0.7380(40) &           1.0158(41) &            1.465(20) \\
    $\DK$ &       ETMC 17 &  0.765(31) &            0.979(19) &            1.336(54) \\
   \hline
    $\DsK$ &     FNAL/MILC & 0.6307(20) &           0.9843(18) &            1.576(13) \\
\hline
\end{tabular}



==> D-meson_semileptonic_decays_with_highly_improved_staggered_quarks/Tables/physical_point_inputs.tex <==
\begin{tabular}{l  l  l}
\hline \hline
Quantity    & Value                     & Reference \\
\hline
$f_\pi$     & $130.2(8) \MeV$           & Ref.~\cite{Aoki:2021kgd}\\
$M_{\pi^0}$ & $134.9768(5) \MeV$        & Ref.~\cite{ParticleDataGroup:2020ssz}\\
$M_{K^0}$   & $497.611(13) \MeV$        & Ref.~\cite{ParticleDataGroup:2020ssz}\\
% $M_{D^0}$   & $1864.83(05) \MeV$        & Ref.~\cite{ParticleDataGroup:2020ssz}\\
% $M_{D_s}$   & $1968.34(07) \MeV$        & Ref.~\cite{ParticleDataGroup:2020ssz}\\
$w_0$       & $0.17177(67) \fm$          & Ref.~\cite{Aoki:2021kgd}\\
\hline
$M_{D^0}$   & $1864.83(05) \MeV$        & Ref.~\cite{ParticleDataGroup:2020ssz}\\
$M_{D_s}$   & $1968.34(07) \MeV$        & Ref.~\cite{ParticleDataGroup:2020ssz}\\
%$m_{l,{\rm \overline{MS}}}(2 \GeV)$
%            &  $3.402(25) \MeV$         & Ref.~\cite{FermilabLattice:2018est}\\
\hline \hline
\end{tabular}


==> D-meson_semileptonic_decays_with_highly_improved_staggered_quarks/Tables/pole_locations.tex <==
\begin{tabular}{cc cccccc}
    \hline\hline
    Decay     & $c\to x$ & $J^P$ & $D_x^*(J^P)$ & $D_y$ & $L$ & $\Delta_{xy,P}$           & 
    $ (\Delta_{xy,P})^{\rm PDG}$ \\
    \hline
    $\Dpi$ & $c\to l$ & $1^-$ & $D^*$           & $D$   & $\pi$    & $\Delta_{ll,+/\perp}$     & $140\MeV$ \\
           &          & $0^+$ & $D^*_0(2300)$   & $D$   & $\pi$    & $\Delta_{ll,0/\parallel}$ & $480\MeV$ \\
    \hline
    $\DsK$& $c\to l$ & $1^-$ & $D^*$            & $D_s$ & $\pi$    & $\Delta_{ls,+/\perp}$     & $-25\MeV$ \\
          &          & $0^+$ & $D^*_0(2300)$    & $D_s$ & $\pi$    & $\Delta_{ls,0/\parallel}$ & $300\MeV$ \\
    \hline
    $\DK$ & $c\to s$ & $1^-$ & $D_s^*$          & $D$   & $K$      & $\Delta_{sl,+/\perp}$     & $200\MeV$ \\
          &          & $0^+$ & $D_{s0}^*(2317)$ & $D$   & $K$      & $\Delta_{sl,0/\parallel}$ & $440\MeV$ \\
    \hline\hline
\end{tabular}

==> D-meson_semileptonic_decays_with_highly_improved_staggered_quarks/Tables/priors_2pt3pt.tex <==
\begin{tabular}{cc c }
\hline\hline
Momentum    & Quantity & Prior value \\
\hline
$\bm{p}^2=0$ & Energy & $M_{\rm 2pt} \pm 10\times \delta M_{\rm 2pt}$\\
     & Amplitude & $A_{\rm 2pt} \pm 10\times \delta A_{\rm 2pt}$\\
\hline
$\bm{p}^2>0$ & Energy & $E_{\rm 2pt}\times\left(1 \pm \alpha_s a^2 \bm{p}^2\right)$ \\
    & Amplitude & $A_{\rm 2pt} \sqrt{M_{\rm 2pt}/E_{\rm 2pt}} \times \left( 1 \pm \alpha_s a^2 \bm{p}^2 \right)$ \\
\hline\hline
\end{tabular}

==> D-meson_semileptonic_decays_with_highly_improved_staggered_quarks/Tables/systematics_breakdown.tex <==
% \begin{tabular}{l | cc | cc | cc}
% \hline \hline
% Source  &   $f_+^{\Dpi}(0)$ & $f_+^{\Dpi}(q^2_{\rm max})$   & $f_+^{\DK}(0)$ & $f_+^{\DK}(q^2_{\rm max})$ & $f_+^{\DsK}(0)$ & $f_+^{\DsK}(q^2_{\rm max})$\\
% \hline
% Chiral-continuum fit & 0.87 & 1.84 & 0.49 & 1.29 & 0.46 & 0.99\\
% \qquad (Statistics $f_\perp$) & (0.21) & (1.46) & (0.07) & (0.95) & (0.07) & (0.73)\\
% \qquad (Statistics $f_0$) & (0.70) & (0.39) & (0.39) & (0.36) & (0.29) & (0.18)\\
% \qquad (Continuum $w_0$) & (0.31) & (0.09) & (0.24) & (0.14) & (0.32) & (0.27)\\
% \qquad (Chiral EFT $f_\perp$) & (0.12) & (0.46) & (0.03) & (0.50) & (0.03) & (0.39)\\
% \qquad (Chiral EFT $f_0$) & (0.24) & (0.13) & (0.11) & (0.14) & (0.05) & (0.03)\\
% \qquad (Discretization $f_\perp$) & (0.08) & (0.73) & (0.06) & (0.41) & (0.03) & (0.41)\\
% \qquad (Discretization $f_0$) & (0.05) & (0.02) & (0.02) & (0.02) & (0.00) & (0.00)\\
% \qquad ($f_\pi^{\rm PDG}$) & (0.16) & (0.10) & (0.06) & (0.04) & (0.12) & (0.04)\\
% \qquad (Meson masses PDG)       & --- & --- & --- & --- & --- & --- \\
% Finite volume          & --- & --- & --- & --- & --- & --- \\
% Topological charge     & --- & --- & --- & --- & --- & --- \\
% \hline
% Total error & 0.87 & 1.84 & 0.49 & 1.29 & 0.46 & 0.99\\
% \hline \hline
% \end{tabular}

\begin{tabular}{l | ccc | ccc | ccc}
\hline \hline
Decay   & $\Dpi$ & & & $\DK$ & & & $\DsK$ & & \\
\hline
Source  & $f_+(0)$ & $f_+(q^2_{\rm max})$ & $f_0(q^2_{\rm max})$   
        & $f_+(0)$ & $f_+(q^2_{\rm max})$ & $f_0(q^2_{\rm max})$   
        & $f_+(0)$ & $f_+(q^2_{\rm max})$ & $f_0(q^2_{\rm max})$\\
\hline
%Chiral-continuum fit & 0.87 & 1.84 & 0.48 & 0.49 & 1.29 & 0.28 & 0.46 & 0.99 & 0.30\\
Statistics $f_\perp$ & 0.21 & 1.46 & 0.01 & 0.07 & 0.95 & 0.01 & 0.07 & 0.73 & 0.02\\
Statistics $f_0$ & 0.70 & 0.39 & 0.40 & 0.39 & 0.36 & 0.22 & 0.29 & 0.18 & 0.12\\
Ctm. $w_0$ & 0.31 & 0.09 & 0.15 & 0.24 & 0.14 & 0.17 & 0.32 & 0.27 & 0.27\\
$\chi$EFT $f_\perp$ & 0.12 & 0.46 & 0.01 & 0.03 & 0.50 & 0.00 & 0.03 & 0.39 & 0.01\\
$\chi$EFT $f_0$ & 0.24 & 0.13 & 0.13 & 0.11 & 0.14 & 0.05 & 0.05 & 0.03 & 0.02\\
Discr. $f_\perp$ & 0.08 & 0.73 & 0.00 & 0.06 & 0.41 & 0.01 & 0.03 & 0.41 & 0.01\\
Discr. $f_0$ & 0.05 & 0.02 & 0.07 & 0.02 & 0.02 & 0.02 & 0.00 & 0.00 & 0.01\\
$f_\pi^{\rm PDG}$ & 0.16 & 0.10 & 0.13 & 0.06 & 0.04 & 0.03 & 0.12 & 0.04 & 0.09\\
%PDG masses        & $\lesssim 0.01$ & --- & --- & --- & --- & --- & --- & --- & ---\\
%Finite volume          & --- & --- & --- & --- & --- & --- & --- & --- & ---\\
%Topo. charge     & --- & --- & --- & --- & --- & --- & --- & --- & ---\\
\hline
Total error & 0.87 & 1.84 & 0.48 & 0.49 & 1.29 & 0.28 & 0.46 & 0.99 & 0.30\\
\hline \hline
\end{tabular}

==> D-meson_semileptonic_decays_with_highly_improved_staggered_quarks/Tables/vcx_summary.tex <==
\begin{tabular}{lllll}
\hline\hline
       &              Process &      Method &      $\Vcx$ & $\Vcx$ (no QED) \\
\hline
$\Vcd$ &    $D\to\pi e^+ \nu$ & $z$-expansion &  0.2251(30) &      0.2251(20) \\
$\Vcd$ &    $D\to\pi e^+ \nu$ &      binned &  0.2250(31) &      0.2250(21) \\
$\Vcd$ &  $D\to\pi \mu^+ \nu$ & $z$-expansion &  0.2199(35) &      0.2199(27) \\
$\Vcd$ &  $D\to\pi \mu^+ \nu$ &      binned &  0.2209(36) &      0.2209(28) \\
$\Vcd$ & $D\to\pi \ell^+ \nu$ & $z$-expansion &  0.2238(29) &      0.2238(19) \\
$\Vcd$ & $D\to\pi \ell^+ \nu$ &      binned &  0.2238(30) &      0.2238(19) \\
$\Vcd$ & $D\to\pi \ell^+ \nu$ &    endpoint &  0.2243(41) &      0.2243(34) \\
\hline
$\Vcs$ &     $D\to K e^+ \nu$ & $z$-expansion & 0.9653(110) &      0.9653(53) \\
$\Vcs$ &     $D\to K e^+ \nu$ &      binned & 0.9631(113) &      0.9631(58) \\
$\Vcs$ &   $D\to K \mu^+ \nu$ & $z$-expansion & 0.9537(111) &      0.9537(56) \\
$\Vcs$ &   $D\to K \mu^+ \nu$ &      binned & 0.9543(116) &      0.9543(65) \\
$\Vcs$ &  $D\to K \ell^+ \nu$ & $z$-expansion & 0.9589(108) &      0.9589(49) \\
$\Vcs$ &  $D\to K \ell^+ \nu$ &      binned & 0.9582(110) &      0.9582(54) \\
$\Vcs$ &  $D\to K \ell^+ \nu$ &    endpoint & 0.9549(110) &      0.9549(61) \\
\hline
$\Vcd$ &   $D_s\to K e^+ \nu$ & $z$-expansion & 0.2582(155) &     0.2582(153) \\
$\Vcd$ &   $D_s\to K e^+ \nu$ &      binned & 0.2583(157) &     0.2583(155) \\
\hline\hline
\end{tabular}



==> D-meson_semileptonic_decays_with_highly_improved_staggered_quarks/results_macros.tex <==
\newcommand{\VcdMuonic}{\ensuremath{0.2199(22)^{\rm Expt}(15)^{\rm QCD}(04)^{\rm EW}(02)^{\rm SIB}[22]^{\rm QED}}}
\newcommand{\VcdCombined}{\ensuremath{0.2238(11)^{\rm Expt}(15)^{\rm QCD}(04)^{\rm EW}(02)^{\rm SIB}[22]^{\rm QED}}}
\newcommand{\VcdFinal}{\VcdCombined}
\newcommand{\VcsElectronic}{\ensuremath{0.9653(28)^{\rm Expt}(40)^{\rm QCD}(15)^{\rm EW}(05)^{\rm SIB}[97]^{\rm QED}}}
\newcommand{\VcsMuonic}{\ensuremath{0.9537(31)^{\rm Expt}(43)^{\rm QCD}(15)^{\rm EW}(05)^{\rm SIB}[95]^{\rm QED}}}
\newcommand{\VcsCombined}{\ensuremath{0.9589(23)^{\rm Expt}(40)^{\rm QCD}(15)^{\rm EW}(05)^{\rm SIB}[95]^{\rm QED}}}
\newcommand{\VcsFinal}{\VcsCombined}
\newcommand{\VcdElectronicDsK}{\ensuremath{0.258(15)^{\rm Expt}(01)^{\rm QCD}[03]^{\rm QED}}}
\newcommand{\VcdFinalDsK}{\VcdElectronicDsK}

==> Tables/d2x_zexpansion_correlations.tex <==
\begin{tabular}{ccccccc ccccccc ccccccc}
$\Dpi$ & & & & & & & $\DK$ & & & & & & & $\DsK$ & & & & & & & \\
$a_0 \equiv b_0$ & $a_1$ & $a_2$ & $a_3$ & $b_1$ & $b_2$ & $b_3$ &$a_0 \equiv b_0$ & $a_1$ & $a_2$ & $a_3$ & $b_1$ & $b_2$ & $b_3$ &$a_0 \equiv b_0$ & $a_1$ & $a_2$ & $a_3$ & $b_1$ & $b_2$ & $b_3$\\
\hline
$1.0000$ & $0.5670$ & $0.5189$ & $-0.2018$ & $0.7547$ & $0.3473$ & $0.0861$ & $0.3219$ & $0.0497$ & $0.0635$ & $-0.0439$ & $0.1897$ & $0.1158$ & $-0.0540$ & $0.2342$ & $0.1305$ & $0.1157$ & $-0.0273$ & $0.1810$ & $0.1459$ & $0.1002$\\
 & $1.0000$ & $0.8912$ & $-0.2826$ & $0.5148$ & $0.2529$ & $0.0747$ & $0.1159$ & $0.0559$ & $0.1385$ & $-0.1328$ & $0.1625$ & $0.1704$ & $-0.1148$ & $-0.0037$ & $0.4332$ & $0.3713$ & $0.0198$ & $-0.0341$ & $-0.0351$ & $-0.0284$\\
 &  & $1.0000$ & $-0.1482$ & $0.5082$ & $0.2782$ & $0.1162$ & $0.1313$ & $0.0438$ & $0.1916$ & $-0.0885$ & $0.2166$ & $0.2197$ & $-0.0308$ & $0.0350$ & $0.2987$ & $0.2781$ & $0.0601$ & $-0.0071$ & $-0.0297$ & $-0.0325$\\
 &  &  & $1.0000$ & $-0.1728$ & $-0.0496$ & $0.0354$ & $-0.0115$ & $-0.0907$ & $0.0014$ & $0.2782$ & $0.0787$ & $0.1182$ & $0.0639$ & $0.0529$ & $0.0228$ & $0.0638$ & $0.1488$ & $0.0634$ & $-0.0154$ & $-0.0969$\\
 &  &  &  & $1.0000$ & $0.8277$ & $0.6066$ & $0.1858$ & $0.1995$ & $0.1837$ & $-0.1531$ & $0.1637$ & $0.1608$ & $0.0996$ & $0.2393$ & $0.0457$ & $0.0571$ & $0.0266$ & $0.2161$ & $0.1520$ & $0.0425$\\
 &  &  &  &  & $1.0000$ & $0.9442$ & $0.0846$ & $0.2589$ & $0.2257$ & $-0.1766$ & $0.1439$ & $0.1970$ & $0.2436$ & $0.1943$ & $0.0190$ & $0.0411$ & $0.0403$ & $0.1979$ & $0.1480$ & $0.0299$\\
 &  &  &  &  &  & $1.0000$ & $0.0226$ & $0.2597$ & $0.2111$ & $-0.1572$ & $0.1088$ & $0.1743$ & $0.2784$ & $0.1524$ & $0.0032$ & $0.0261$ & $0.0512$ & $0.1659$ & $0.1280$ & $0.0200$\\
 &  &  &  &  &  &  & $1.0000$ & $-0.0332$ & $0.0747$ & $-0.0201$ & $0.7753$ & $0.4920$ & $-0.0189$ & $0.2613$ & $0.1817$ & $0.1423$ & $-0.1223$ & $0.1642$ & $0.0590$ & $-0.0293$\\
 &  &  &  &  &  &  &  & $1.0000$ & $0.3272$ & $-0.1586$ & $-0.0909$ & $-0.1090$ & $0.0420$ & $0.0715$ & $0.0236$ & $-0.0442$ & $-0.1656$ & $0.0458$ & $0.0377$ & $0.0266$\\
 &  &  &  &  &  &  &  &  & $1.0000$ & $-0.7543$ & $0.2071$ & $0.2565$ & $0.1457$ & $-0.0938$ & $0.1078$ & $0.0219$ & $-0.2929$ & $-0.1126$ & $-0.1094$ & $-0.0790$\\
 &  &  &  &  &  &  &  &  &  & $1.0000$ & $-0.0594$ & $-0.1119$ & $-0.2259$ & $0.1727$ & $-0.0470$ & $0.0700$ & $0.3279$ & $0.1515$ & $0.0836$ & $-0.0062$\\
 &  &  &  &  &  &  &  &  &  &  & $1.0000$ & $0.9087$ & $0.1012$ & $0.2751$ & $0.2429$ & $0.2479$ & $-0.0663$ & $0.1986$ & $0.0374$ & $-0.1217$\\
 &  &  &  &  &  &  &  &  &  &  &  & $1.0000$ & $0.2126$ & $0.2038$ & $0.2315$ & $0.2517$ & $-0.0060$ & $0.1481$ & $-0.0029$ & $-0.1604$\\
 &  &  &  &  &  &  &  &  &  &  &  &  & $1.0000$ & $-0.1959$ & $-0.1108$ & $-0.0868$ & $0.1128$ & $-0.1256$ & $-0.0562$ & $0.0179$\\
 &  &  &  &  &  &  &  &  &  &  &  &  &  & $1.0000$ & $0.1825$ & $0.2612$ & $-0.0266$ & $0.8467$ & $0.5197$ & $0.0973$\\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  & $1.0000$ & $0.9274$ & $-0.2432$ & $0.1899$ & $0.1915$ & $0.1180$\\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & $1.0000$ & $-0.0514$ & $0.3243$ & $0.3065$ & $0.1764$\\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & $1.0000$ & $-0.0551$ & $-0.1580$ & $-0.2098$\\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & $1.0000$ & $0.8344$ & $0.4260$\\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & $1.0000$ & $0.8442$\\
 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & $1.0000$\\
\end{tabular}

